Find or Classify? Dual Strategy for Slot-Value Predictions on Multi-Domain Dialog State Tracking

Dialog state tracking (DST) is a core component in task-oriented dialog systems. Existing approaches for DST mainly fall into one of two categories, namely, ontology-based and ontology-free methods. An ontology-based method selects a value from a candidate-value list for each target slot, while an ontology-free method extracts spans from dialog contexts. Recent work introduced a BERT-based model to strike a balance between the two methods by pre-defining categorical and non-categorical slots. However, it is not clear enough which slots are better handled by either of the two slot types, and the way to use the pre-trained model has not been well investigated. In this paper, we propose a simple yet effective dual-strategy model for DST, by adapting a single BERT-style reading comprehension model to jointly handle both the categorical and non-categorical slots. Our experiments on the MultiWOZ datasets show that our method significantly outperforms the BERT-based counterpart, finding that the key is a deep interaction between the domain-slot and context information. When evaluated on noisy (MultiWOZ 2.0) and cleaner (MultiWOZ 2.1) settings, our method performs competitively and robustly across the two different settings. Our method sets the new state of the art in the noisy setting, while performing more robustly than the best model in the cleaner setting. We also conduct a comprehensive error analysis on the dataset, including the effects of the dual strategy for each slot, to facilitate future research.

==> discussion.tex <==


\section{Open Discussion} \label{discussion}
% Moreover, with the recent release of the MultiWOZ 2.0 \cite{budzianowski2018multiwoz} and it later update  MultiWOZ 2.1 \cite{eric2019multiwoz} datasets. Multi-domain dialog state tracking, which enhances task-oriented dialog systems to handle tasks across different domains and support large number of services, are gradually becoming popular and important. 
With the recent release of MultiWOZ 2.0 \cite{budzianowski2018multiwoz} and its later update MultiWOZ 2.1 \cite{eric2019multiwoz}, multi-domain dialog state tracking is enjoying popularity in enhancing task-oriented dialog systems, handling tasks across different domains and supporting large number of services.
% Compared with several complicated datasets and standard leaderboards in text reading comprehensions \cite{chen2018neural}, only two large task-oriented multi-domain dialogue corpora to-date and are recently released \cite{eric2019multiwoz, rastogi2019towards}. 
% Another easy-ignored but important problem is there are no standard ways to handle the MultiWOZ dataset, where the test set are usually modified based on pre-processing ways, and these ways are either different or not mentioned in the papers \cite{rastogi2019towards,goel2019hyst,gao2019dialog,lee2019sumbt}, and some results are manually  collected to the website \footnote{http://dialogue.mi.eng.cam.ac.uk/index.php/corpus/}. easily-ignored but important
However, a potential problem is that no standard ways are available to handle the MultiWOZ dataset; the test set are usually modified based on different pre-processing ways.
For example, \cite{wu2019transferable} fixes general label errors for the  dataset,\footnote{\url{https://github.com/jasonwu0731/trade-dst/blob/master/utils/fix_label.py}} and \cite{lee2019sumbt} treats all the slot-value labels in the  dataset not appeared in the ontology as \textit{none}.\footnote{see  $\texttt{convert\_to\_glue\_format.py}$ under the \\
\url{https://github.com/SKTBrain/SUMBT/blob/master/data/multiwoz/original.zip}
}
% are either different or not clearly mentioned in the papers \cite{rastogi2019towards,goel2019hyst,gao2019dialog,lee2019sumbt}. 
% In addition, some results are manually collected to the website \footnote{http://dialogue.mi.eng.cam.ac.uk/index.php/corpus/}. 
% As there are annotation errors of around $40\%$ turns in MultiWOZ 2.0 \cite{eric2019multiwoz} dataset and more than $30\%$ of turns in MultiWOZ 2.1 dataset based on our own statistics, slightly modification for test set could make a difference. 
Moreover, there are around $40\%$ of annotation errors of turns in the MultiWOZ 2.0 dataset as reported in \cite{eric2019multiwoz}, and more than $30\%$ of that in the MultiWOZ 2.1 dataset from our  statistics, hence even slight modifications on the test set would make a difference. 
% To facilitate the research on multi-domain dialog state tracking on task-oriented dialog systems, we will build a leaderboard for MultiWOZ 2.1 dataset \footnote{more detailes can be found in...}.
To make fair comparisons and facilitate the research on multi-domain dialog state tracking in task-oriented dialog systems, it is important to have the standard way to handle the test set and the evaluation process. 
%build a standard benchmark test set. 

% Besides, 
% Wizard-of-Oz ways to build benchmark datasets often leads to different errors, e.g., annotation errors, unmatched states across turns, while DST has a high request for the dataset quality as the error could be accumulated during dialog state tracking process. Hence it is also important to think ways on how to build DST datasets. 

% for MultiWOZ 2.1 dataset \footnote{more detailes can be found in...}.


==> misc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{llll}
\hline
\textbf{Slot Name}     & \textbf{DS-Span} & \textbf{DS-DST} & \textbf{DS-Picklist} \\ \hline
hotel-type             & 86.83            & 93.97 (\textbf{+7.14})   & 94.29 (\textbf{+7.46})        \\
attraction-name        & 90.76            & 93.81 (\textbf{+3.05})   & 93.93 (\textbf{+3.17})        \\
hotel-internet         & 91.10            & 97.48 (\textbf{+6.38})   & 97.26 (\textbf{+6.16})        \\
hotel-parking          & 92.21            & 97.18 (\textbf{+4.97})   & 96.99 (\textbf{+4.78})        \\
restaurant-name        & 92.90            & 93.38 (+0.48)   & 92.89 (-0.01)        \\
hotel-name             & 93.46            & 94.87 (\textbf{+1.41})   & 94.77 (\textbf{+1.31})        \\
attraction-type        & 93.99            & 96.86 (\textbf{+2.87})   & 96.91 (\textbf{+2.92})        \\
hotel-area             & 95.24            & 95.87 (+0.63)   & 95.47 (+0.23)        \\
restaurant-area        & 96.16            & 96.86 (+0.70)   & 97.18 (\textbf{+1.02})        \\
attraction-area        & 96.20            & 96.96 (+0.76)   & 96.73 (+0.53)        \\
hotel-price range      & 96.81            & 97.39 (+0.58)   & 96.97 (+0.16)        \\
restaurant-food        & 97.03            & 97.60 (+0.57)   & 97.19 (+0.16)        \\
restaurant-price range & 97.05            & 97.73 (+0.68)   & 97.69 (+0.64)        \\
hotel-stars            & 97.43            & 97.48 (+0.05)   & 97.76 (+0.33)        \\
train-departure        & 97.45            & 98.55 (\textbf{+1.10})   & 98.34 (\textbf{+0.89})        \\
taxi-departure         & 97.71            & 98.53 (\textbf{+0.82})   & 98.59 (\textbf{+0.88})        \\
train-destination      & 97.84            & 98.86 (\textbf{+1.02})   & 98.59 (\textbf{+0.75})        \\
taxi-destination       & 98.06            & 98.49 (+0.43)   & 98.24 (+0.18)        \\
train-day              & 99.23            & 99.35 (+0.12)   & 99.33 (+0.10)        \\
hotel-book day         & 99.32            & 99.32 (+0.00)   & 99.24 (-0.08)        \\
restaurant-book day    & 99.35            & 99.57 (+0.22)   & 99.44 (+0.09)        \\ \hdashline
train-leave at         & 93.66            & 93.30 (-0.36)   & 93.91 (+0.25)        \\
train-arrive by        & 95.58            & 95.78 (+0.20)   & 96.59 (\textbf{+1.01})        \\
train-book people      & 98.00            & 97.84 (-0.16)   & 98.51 (+0.51)        \\
restaurant-book time   & 98.64            & 98.44 (-0.20)   & 99.04 (+0.40)        \\
taxi-leave at          & 98.76            & 98.53 (-0.23)   & 98.94 (+0.18)        \\
hotel-book people      & 98.94            & 99.04 (+0.10)   & 99.29 (+0.35)        \\
taxi-arrive by         & 99.09            & 99.01 (-0.08)   & 99.09 (+0.00)        \\
hotel-book stay        & 99.28            & 99.25 (-0.03)   & 99.40 (+0.12)        \\
restaurant-book people & 99.32            & 99.16 (-0.16)   & 99.44 (+0.12)        \\ \hdashline
Average Accuracy & 96.25\% & 97.35\% & 97.40\% \\ \hline
\end{tabular}}\caption{Slot accuracy on the test set of the MultiWOZ 2.1. `+/-' indicates absolute performance improvement/degradation compared with DS-Span, where performances improvement which are significant based on bootstrapping re-sampling (p<0.05) are highlighted in bold. The slots above the first dashed line are picklist-based slots and the slots below the first dashed line are span-based slots for DS-DST. The last row shows the average slot accuracy.} \label{table:per-slot-acc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}%[t]
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lll}
\hline
\textbf{Models}      & \textbf{\begin{tabular}[c]{@{}l@{}}MultiWOZ 2.0\\ (Joint Acc.)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}MultiWOZ 2.1\\ (Joint Acc.)\end{tabular}} \\ \hline
SpanPtr   \cite{xu2018end}           & 30.28\%                                                                     & 29.09\%                                                                     \\
Ptr-DST        &- & 42.17\%                 \\

GLAD   \cite{zhong2018global}              & 35.57\%                                                                     &                 -                                                            \\
%TSCP   \cite{lei2018sequicity}              & 39.24\%                                                                     &                 37.12\%                                                            \\
FJST     \cite{eric2019multiwoz}            & 40.20\%                                                                     & 38.00\%                                                                     \\
HJST      \cite{eric2019multiwoz}         & 38.40\%                                                                     & 35.55\%                                                                     \\
HyST (single)   \cite{goel2019hyst}     & 42.33\%                                                                     & -                                                                      \\
HyST (ensemble)   \cite{goel2019hyst}     & 44.24\%                                                                     & 38.10\%$^{\star}$                                                                      \\
DSTreader (single) \cite{gao2019dialog}  & 39.41\%                                                                     & 36.40\%$^{\star}$                                                                     \\
DSTreader (ensemble)\cite{gao2019dialog} & 42.12\%                                                                     & -                                                                           \\
TRADE   \cite{wu2019transferable}             & 48.62\%                                                                     & 45.60\%$^{\star}$                                                                     \\
SUMBT \cite{lee2019sumbt} & 46.65\% & - \\ 
COMMER   \cite{ren2019scalable}            & 45.72\%                                                                     & -                                                                           \\
ZSDST \cite{rastogi2019towards}              & 51.60\%                                                                     & 48.90\%                                                                     \\ \hline
DS-Span              & \multicolumn{1}{l}{42.59\%}                                                        & \multicolumn{1}{l}{40.00\%}                                                        \\
DS-DST               & \multicolumn{1}{l}{52.24\%}                                                        & \multicolumn{1}{l}{51.21\%}                                                        \\
DST-Picklist         &  \multicolumn{1}{l}{\textbf{54.39\%}}                                                        &  \multicolumn{1}{l}{\textbf{53.30\%}}                                                        \\ \hline
\end{tabular}}
\caption{Joint accuracy on the test set of MultiWOZ 2.0 and MultiWOZ 2.1. $^{\star}$: reported by \cite{eric2019multiwoz}.} \label{table-jointacc}
\vspace{-1em}
\end{table*}
